Building Prior Knowledge: A Markov Based Pedestrian Prediction Model Using Urban Environmental Data

Autonomous Vehicles navigating in urban areas have a need to understand and predict future pedestrian behavior for safer navigation. This high level of situational awareness requires observing pedestrian behavior and extrapolating their positions to know future positions. While some work has been done in this field using Hidden Markov Models (HMMs), one of the few observed drawbacks of the method is the need for informed priors for learning behavior. In this work, an extension to the Growing Hidden Markov Model (GHMM) method is proposed to solve some of these drawbacks. This is achieved by building on existing work using potential cost maps and the principle of Natural Vision. As a consequence, the proposed model is able to predict pedestrian positions more precisely over a longer horizon compared to the state of the art. The method is tested over "legal" and "illegal" behavior of pedestrians, having trained the model with sparse observations and partial trajectories. The method, with no training data, is compared against a trained state of the art model. It is observed that the proposed method is robust even in new, previously unseen areas.

==> sections/related_work.tex <==
\section{Related Work} \label{related_work}

Related work can broadly be classified into learning problems, where pedestrian behaviour is learnt based on observations and their future states are inferred from these models. They can further be classified into environment based and non environment based methods. Environment based methods like Kitani, Ziebart and Vasquez. Non environment based ones like < Find one>, <Dizan's paper> and <luis merino's paper>. Specifically, we talk about the state of the art in < luis merino's paper>. This uses the principle of GHMMs set out in <Dizan's paper>

A GHMM, the growing hidden markov model, is called so because the topology of the HMM grows with new observations. The method, called the Instantaneous topological model (ITM) [reference for ITM here] is used to build the topolgy. The states of the HMM are created by extending the generated nodes with goals. In <luis' paper>, goals are discovered, added or removed from a list which are used to create the extended states containing the node position of the created ITM node and associated with all the discovered goals. Learning the parameters of the model is done based on observed partial trajectories. Learning is performed by using a form of the EM called the incremental Baum Welch algorithm. The learnt parameters, A, B and $\pi$ are then used to perform inference and predict pedestrian goals and future positions. The state of the art has the following issues: 

\begin{itemize}
	\item \textit{Default priors}: When a node on the ITM is created, the corresponding state is created with a default prior. 
	\item \textit{Offline inference}: Both methods begin the learning process only after the last observation in the trajectory. 
	\item \textit{Rich datasets}: For the ITM to grow and create a topology covering the entire observed environment, a rich dataset with many trajectories is required. The methods cannot be applied for sparse datasets.
	\item \textit{Default transition values}: When a node is created using the ITM method, the nodes closest to it are connected bidirectionally with a default probability. 
	\item \textit{Unaccounted occlusions}: Neither method takes into account semi-dynamic obstacles that can occlude a few nodes on the topology for a short period of time. 
\end{itemize}

This work extends the state of the art to solve most of the issues described above. The contributions of this work is the extension of the GHMM method to take into account temporary occlusions in the environment and to solve the issue of sparse, untagged observations in a previously unseen environment. This work can be used to predict pedestrian behaviour in urban areas where temporary occlusions can exist in the form of a slow moving car or car stopped at a traffic light for a short period of time. These elements change the behaviour of pedestrians in the environment, which we hope to capture and predict with our method. 

